The Theory of Spin Noise Spectroscopy: A Review

Direct measurements of spin fluctuations are becoming the mainstream approach for studies of complex condensed matter, molecular, nuclear, and atomic systems. This review covers recent progress in the field of optical Spin Noise Spectroscopy (SNS) with an additional goal to establish an introduction into its theoretical foundations. Various theoretical techniques that have been recently used to interpret results of SNS measurements are explained alongside with examples of their applications.

==> Sections123_17.tex <==
\section{Introduction}


In experimental measurements, the noise  is not necessarily a
complication. From noise, one can often extract  valuable
information regarding its sources.
Consider, for example, the circuit in Fig.~\ref{fig1_1}(a) containing a resistor and battery.
The standard way of measuring the resistance $R$ is by application of a constant voltage $V$ to the resistor and the measurement of average electric current, $I$. The resistance is then given by
$R=V/I$. The noise-based measurement is a less invasive approach.
It was shown as early as in 1928 \cite{Johnson28a,Nyquist28a} that
the resistance  can be found from voltage
fluctuations at the thermodynamic equilibrium (the Johnson-Nyquist
noise \cite{Johnson28a,Nyquist28a})  without application of any
external voltage (see Fig.~\ref{fig1_1}(b) circuit). Indeed, the fluctuation dissipation theorem states
that the voltage variance (mean square) per Hertz of the bandwidth, is
given by  \cite{ft2,ft3}
\begin{equation}
 \langle V^2\rangle=4k_B TR,	
 \label{noise1}
 \end{equation}
 where $k_B$ is the Boltzmann constant, $T$ is temperature, and the
 average is taken over many repeated measurements. Equation~(\ref{noise1})
can be used to find the resistance $R$ from measured voltage fluctuations and
known temperature.

\begin{figure}[b]
\centerline{\includegraphics[width=0.75\columnwidth]{fig1_1.pdf}}
\caption{Circuits for (a) standard and (b) noise measurements of the resistance $R$. Here, A is the ammeter measuring the average current $I$ and V is the voltmeter measuring voltage fluctuations $V(t)$. The constant voltage $V$ across the battery in ($a$) is known.
}
\label{fig1_1}
\end{figure}

The above example shows that by studying  equilibrium
fluctuations we are able to obtain a single characteristic of a
circuit component. However, we can achieve much more. By measuring higher
correlators of noise (e.g., averages of higher powers of $V$) or by measuring the
noise in a nonequilibrium regime, one can avoid restrictions imposed by
the fluctuation-dissipation theorem and obtain the most detailed description
of electron interactions \cite{shot-noise-rev,nazarov-book,levitov-rev}.
For example, let's consider the case when the applied voltage induces
a current, $I$, with mean and variance, $\langle I \rangle$ and
var$(I) = \langle I^2 \rangle - \langle I \rangle^2$, respectively. The variance can be split
into the equilibrium and nonequilibrium parts, var($I$)=var($I$)$_{eq}$+var($I$)$_{neq}$.
The nonequilibrium part carries considerable
information about the physics of electrons. In particular, if
electrons combine into quasiparticles of charge $e^*$, then the ratio of the
nonequilibrium variance to mean is proportional to $e^*$, i.e. var($I$)$_{neq}$/
$\langle I  \rangle \sim e^*$ \cite{shot-noise-rev}.  This observation was used in practice
to obtain the long-sought experimental proof of the fact that the
quasiparticles in the fractional quantum Hall effect have fractional
charges \cite{4,5}.

Unfortunately, the charge current noise has been very hard to study
because of multiple parasitic effects induced, e.g., by contacts with leads, measurement devices, etc.
The proof of the fractional charge of anyons is one of only a few transformative experimental results in the field of electron counting statistics, while theoretical developments were much more promising. Among them are predictions of new types of quantum phase transitions in rare fluctuations \cite{fcs-qpt}, approaches to measure the  quantum entanglement entropy \cite{klich1} and qubit states \cite{8}, and results in the area of full counting statistics of strongly correlated electron states \cite{9,nazarov-rev}.

\begin{figure}[b]
\centerline{\includegraphics[width=0.75\columnwidth]{fig1_2noise}}
\caption{ Faraday rotation noise signal in real time.
}
\label{noise-fig1}
\end{figure}

Spin noise spectroscopy (SNS) is an alternative route
to obtain information about dynamics of various systems based on their {\it spin fluctuations}.
This method was introduced in
the pioneering work of Alexandrov and Zapasskii as early as in 1981 \cite{aleksandrov1981magnetic}.
However, it took over two decades of instrumentation progress including
development of real-time fast Fourier transformation (FFT) spectrum
analyzers and ultrafast digitizers before this technique had become
established as a powerful method to study spin dynamics in atomic
gases \cite{noise-nat}, conduction electrons \cite{Oestreich05}, and localized states in semiconductors \cite{Crooker10}. It should be emphasized that currently,
there is a large variety of available optical and non-optical spin noise measurement techniques targeting different applications. Some of the experimental methods, such as the resonance force microscopy  \cite{cantilever-science} and NV-center magnetometry \cite{NV2,NV3,nV1}, have been introduced  only recently and may experience considerable development in the near future.

 In this review, we will focus  on the frequently used optical approach
based on the Faraday rotation spectroscopy, which has a relatively broad range of applications and has been the topic of many theoretical and experimental studies during the last decade.  To illustrate the main idea of this technique, let us consider an ensemble of spins in a small mesoscopic volume of an atomic gas or a semiconductor that contains $N$ atoms or electrons with spins in a constant magnetic field $B$. Statistical fluctuations of $N$ paramagnetic spins should generate spin fluctuations of the order of $\sqrt{N} $, even in a zero magnetic field at equilibrium \cite{noise-nat}. Optically, such fluctuations are measured  by detecting the Faraday rotation (Fig.~\ref{noise-fig}(a))  of the polarization axis of a linearly polarized beam ($\sim$1-100 $\mu$m diameter) passing through a sample
\footnote{Note that the relative fluctuations $\sim \sqrt{N}/N=1/\sqrt{N}$ increase with decreasing the beam diameter.}.
A typical experimental setup is shown in Fig.~\ref{noise-fig1}.

The polarization rotation angle is proportional to the local instantaneous magnetization of the illuminated region and its fluctuations can be traced with sub-nanosecond resolution
in time \cite{high-band,Starosielec08a,gaas2,Hubner13a},
thus providing considerable statistical data about local
magnetization dynamics. The spin noise power spectrum is found as FFT of the autocorrelation function $\la S_z(t) S_z(0) \ra$ (for an example, see Fig.~\ref{noise-fig}(b)). The position and shape of the spin noise
peaks are used to extract physical parameters of a particular system.
Importantly, the frequency of the measurement beam can be detuned from  system resonances  so that dissipative effects during measurements are minimized. Therefore, spin fluctuations can be studied  in spin systems at the thermodynamic equilibrium without inducing undesired extrinsic excitations.
Potentially, this technique can be applied to any material that demonstrates measurable Faraday or Kerr rotations induced by partial spin polarization. These include most known semiconductors, topological insulators, unconventional superconductors, as well as atomic gases.


The research on SNS is highly interdisciplinary with diverse applications in the areas of atomic gases, conduction electrons, spintronics, optoelectronics, semiconductor quantum dots, spin glasses, and  micromagnetics. By itself, SNS essentially differs from the traditional methods used in materials science.  Moreover, the very type of data that SNS deals with is unusual for
condensed matter physics. SNS works with {\it  stochastic signals} that
often have to be processed with a rate of gigabytes per second, sometimes during days or longer \cite{gaas4,instr-rev}.


 Several reviews have been already written about  SNS
with the focus on experimental developments \cite{alexandrov-rev, Zapasskii13b,OestreichPhysE,Oestreich-rise,Oestreich-rev3,glazov-rev}. The goal of the present review is different. Despite diverse applications, there are established theoretical methods and results that can be useful for theorists entering or working in this field.  We wrote our review  to provide an introduction to  SNS from the theoretical point of view  minimizing the discussion of instrumentation. Thus, our main attention is focused on the theoretical justification of the technique, theoretical methods to study spin noise, and the problems  that  will likely benefit from advances in the theory of SNS in the future.

\begin{figure}[t]
\centerline{\includegraphics[width=0.9\columnwidth]{fig2_1_crooker_Rb}}
\caption{SNS of  Rb vapor \cite{noise-nat}: (a)
The experimental setup: a linearly polarized laser beam ($\sim$1-100 $\mu$m diameter) passes through a small volume of gas.
The outgoing beam experiences measurable Faraday rotation of polarization, $\delta \theta_F$,
proportional to the  instantaneous gas magnetization in the volume. (b) The noise power spectrum from Rb vapor showing two peaks from $^{85}$Rb and $^{87}$Rb at corresponding Larmor frequencies. For more details, see Ref. \cite{noise-nat}. Reprinted with permission from Macmillan
Publishers Ltd: Nature 431, pp. 49–52, 2004, Copyright \copyright (2004) \cite{noise-nat}.
}
\label{noise-fig}
\end{figure}

\iffalse
\begin{figure}[t]
\centerline{\includegraphics[width=0.95\columnwidth]{fig1_3SNSsetup}}
\caption{ Experimental setup: a linearly
  polarized laser beam ($\sim$1-50$\mu$m diameter) passes through a slab,
  e.g., of GaAs. The outgoing beam experiences measurable Faraday
  rotation of polarization, $\delta \theta_F$, proportional to the
  instantaneous  magnetization of electrons.  Magneto-optical Faraday
  Rotation (FR) \cite{faraday4,faraday1,faraday2,faraday3} originates
  from different indices of refraction ($n_{R,L}$) for right- and
  left-circularly polarized (RCP/LCP) light, which in turn couples
  selectively to the number of "spin-up" and "spin-down" electrons in
  the system ($N_{\uparrow/\downarrow}$): the FR angle $\theta_F \sim
  N_{\uparrow}-N_{\downarrow}$. Because FR couples to spins via
  $n_{L,R}$ and not via absorption, it can measure spins almost
  without perturbing them. Reprinted figure with permission from S. A. Crooker et al.,
  Physical Review B 79, p. 035208, 2009 \cite{noise-gaas}. Copyright \copyright (2009) by the American Physical Society.
%This method enables 100\% efficient signal averaging of noise power spectra (up from 0.1\% for commercial analyzers), and sub-nanoradian/root-Hz FR noise floors. Note that 1 nanoradian is the angle subtended by the width of a human hair viewed from a distance of 100 km!   "Weak" measurements of this type provide the basis for so-called "quantum non-demolition" measurements, wherein the quantum state being probed is not destroyed by the measurement itself \cite{12}.
  %(b) Measured Lorentzian shape of equilibrium spin noise power
  %spectrum in electron-doped GaAs. Here $\omega_L$ is the Larmor
  %frequency in an external in-plane magnetic field $B_x$, and
  %$\tau_s$ is the spin relaxation time \cite{noise-gaas}. (c) Log-log
  %plot of the  spin noise power spectrum of InGaAs quantum dots
  %\cite{sinitsyn-12prl-1}.
}
\label{SNSsetup}
\end{figure}
\fi

Our review is organized as follows. In Sec.~2, we define various spin correlators and discuss their elementary properties. In Sec.~3, we review available experimental results from the theoretical perspective, illustrating theoretical problems and providing examples of elementary theoretical calculations. Moreover, in order to place the optical SNS into a broader context, subsection~3.5 contains a brief review of several alternative spin noise characterization techniques.
In Sec.~4, we provide quantum theory of spin correlators in the weak measurement framework. Section~5 contains an introduction to the theory of measurement based on the Faraday rotation effect. Section~6 is devoted to sum rules that are applicable practically to all spin systems studied by  SNS. Sections 7-9 review  theoretical  methods  that are frequently used in the research on SNS. Section~10 reviews possible future research directions and extensions of SNS.

Different sections of this review are written at different levels of complexity.
Sections~2-3 set the framework of problems for the rest of the review and provide introduction to the  SNS at a nonspecialist level. Sections~4-7 contain introductions to different  theoretical aspects of the optical SNS with many worked out examples. Although there are occasional cross-references between  these sections, they  are independent of each other and can be read in an arbitrary order. Subsections~8.1 and 8.2 are written in the same style but they should be more accessible to readers  with prior experience in spin drift-diffusion equation and Kubo formula.
In sections~8.3-10, we return to the ``review" mode in order to cover a large variety of other, more specified, theoretical  ideas without attempting to provide a detailed introduction.

%Beyond SNS a correlators similar to $C_3(\omega_1,\omega_2)$ was measured as a function of frequencies only recently to describe the shot noise  of electric charge currents through an artificial nanostructure \cite{fcs-exp4}. Specially engineered nanoscale systems could allow measurements of charge current cumulants in the time domain up to 15th order and the  study  of fundamental nonequilibrium fluctuation relations \cite{fcs-exp1,fcs-exp2,fcs-exp3} but such measurements could not be applied to materials characterization.

\section{Spin Correlators: Definition and Basic Properties}

\subsection{2nd Order Correlator and Noise Power Spectrum}

The simplest characteristic that describes correlations of a signal in SNS is the spin-spin correlator
\begin{equation}
g_2(t_2,t_1)\equiv \la S_z(t_2) S_z(t_1) \ra,
\label{c2-220}
\end{equation}
where $S_z(t)$ is the time-dependent spin polarization in the observation region and $z$ is the measurement axis.
Generally, this correlator is a function of two time arguments, however, if measurements are performed in the steady state then (due to the translation invariance in time) this correlator depends only on the time difference $t$:
\begin{equation}
g_2(t)=\la S_z(t) S_z(0) \ra.
\label{c2-22}
\end{equation}

In many (but not all \cite{real-time-SNS}) experimental setups, it is much more convenient to process signals in the frequency domain.
Let's consider first the straightforward way to calculate the correlator (\ref{c2-22}) from an experimentally measured ``trajectory" $S_z(t)$. In order to obtain (\ref{c2-22}), the total measurement time interval should be divided into relatively long time intervals $T_m \gg \tau_s$, where $\tau_s$ is the characteristic spin relaxation time. Each time interval of size $T_m$ also consists of $N_m \gg 1$ elementary intervals of size $dt \ll \tau_s$. Naively, one may think that in order to obtain (\ref{c2-22}), one should take all pairs of time moments, $t_i$ and $t_{i+j}$, within the same time interval of size $T_m$, and calculate all possible products of measurement results $S_z(t_{i+j})S_z(t_i)$. Then, the average over $i$
provides $\la S_z(t_j) S_z(0) \ra$. Additional averaging over the
 large time intervals of size $T_m$ further increases the precision of calculations.
This straightforward process, however, is not optimal as
$N_m$ measurement points in the interval $T_m$ require the
calculation of  $\sim N_m^2$ products $S_z(t_{j+i})S_z(t_{i})$ in order to estimate correlator (\ref{c2-22}) for all different $t$.
For measurements performed with, e.g.,  a nanosecond resolution,
 continuous data processing imposes very strict
hardware requirements that are difficult to satisfy.

%If measurements are performed with, e.g.,  a nanosecond resolution, then the
%information arrives at the rate of gigabytes per second. In order to secure a
%continuous data processing while avoiding information overflow,
%the physical data should be processed at the same speed.


The widely used approach is based on the Fourier transform of the recorded trajectory during the measurement interval $T_m$
\begin{equation}
a(\omega) =\frac{1}{\sqrt{T_m}} \int\limits_0^{T_m} \textnormal{d}t e^{i\omega t} S_z(t).
\label{aom}
\end{equation}
A typical FFT algorithm (e.g., the Cooley-Tukey FFT algorithm) requires $t\sim N_m {\log}(N_m) \ll N_m^2$ steps to perform. Note that since the measured trajectory $S_z(t)$ is real, $a(-\omega)=a^*(\omega)$. For a system in the steady state, $\la a(\omega)\ra=0$ at
 $\omega \ne 0$, where the average is considered over repeated time intervals of size $T_m$ under  identical experimental conditions~\footnote{Generally, $S_z(t)$ may have a constant component, so that $\la S_z(t)\ra=0$ is not required.}.

 The most accessible physically interesting characteristic in the frequency domain is the {\it  noise power spectrum},  defined as
\begin{equation}
C_2(\omega) = \langle |a(\omega)|^2 \rangle.
\label{noiseP1wk}
\end{equation}
One can easily prove that, due to the translation invariance in time,
$$
\langle a(\omega) a(\omega') \rangle=0, \quad {\rm for} \,\, \omega \ne -\omega'.
$$
It is crucial for fast signal processing that $C_2(\omega)$ depends only on a single argument, so that its calculation for all independent values of $\omega$ scales as $\sim N_m$ for a discretized signal, as desired, so the slowest step in determining $C_2(\omega)$ is application of the FFT algorithm.

Another important property of the noise power spectrum is the additivity, namely, the contributions from independent noise sources add to each other. Indeed, suppose that the measured Fourier transform of the signal is given by $a(\omega) = a_{\rm ph}(\omega) +\zeta(\omega)$, where $a_{\rm ph} (\omega)$ is  the physical spin noise signal and $\zeta(\omega)$ is an uncorrelated from $a_{\rm ph} (\omega)$ background noise that originates, e.g., from an amplifier or represents the photon shot noise. In such a case $\langle a_{\rm ph}(\omega) \zeta(\omega) \rangle = 0$, so
\beq
C_2(\omega) = \la  | a_{\rm ph} (\omega)|^2 \ra +  \la  | \zeta (\omega)|^2 \ra.
\label{backgr}
\eeq
It is possible  then to get rid of the background part by measuring it
separately. The most popular way to do this is to measure the spectrum in a large external magnetic field applied in the transverse
direction to the measurement beam. This field induces fast spin
precessions that  move the physical part of the noise power to very
high frequencies. By measuring the background level in such a field, the
physical noise is obtained by subtracting $\la  | \zeta (\omega)|^2
\ra$ from (\ref{backgr}).


The noise power spectrum is also often easier to interpret than the spin-spin
correlator in  real time. However, if correlators are needed in the
time domain, there is the following important theorem that relates the
noise power spectrum to the time correlator $g_2(t)$:

\underline{\it Wiener-Khinchine theorem} \cite{kogan-book}: In the steady state, the noise power spectrum and the spin-spin correlator are related by the Fourier transform:
\begin{equation}
C_2(\omega)=2 \int\limits_0^{\infty} \textnormal{d}t \cos(\omega t) \la S_z(t) S_z(0) \ra.
\label{c2-1}
\end{equation}
This theorem requires several conditions, such as the requirement that the measurement time is much longer than the spin relaxation time ($T_m \gg \tau_s$), which are discussed in more detail, e.g., in \cite{kogan-book,pecselin-book}.
Apart from these details, the proof is straightforward: Substituting
the definition of the Fourier transformed trajectory (\ref{aom}) into (\ref{noiseP1wk}), and using the property $g_2(t_1,t_2) = g_2(t_1-t_2)$ and the fact that, since $S_z(t)$ is real, $a^*(\omega)=a(-\omega)$,  we  find


\begin{eqnarray}
C_2(\omega) = \frac{1}{T_m} \lim \limits_{T_m \rightarrow \infty} \int\limits_{-T_m/2}^{T_m/2} \textnormal{d}t_1 \int\limits_{-T_m/2}^{T_m/2} \textnormal{d}t_2 \, e^{i\omega (t_1-t_2)} \nonumber \\ \;\;\;\;\;\;\;\;\;\;  \times \la S_z(t_2) S_z(t_1) \ra =  \int\limits_{-\infty}^{\infty } \textnormal{d}t \, e^{i\omega t} \la S_z(t) S_z(0) \ra. \label{proof1}
\end{eqnarray}
Taking into account that $S_z(t)$ is the real valued signal, i.e. it is not an operator, we can use the property $ \la S_z(-t) S_z(0) \ra =  \la S_z(t) S_z(0) \ra$, which demonstrates that the last integral in (\ref{proof1}) coincides with (\ref{c2-1}). This proves the theorem.

\iffalse
\begin{figure}[t]
\centerline{\includegraphics[width=0.9\columnwidth]{fig2_1_crooker_Rb}}
\caption{SNS of  Rb vapor \cite{noise-nat}: {\bf a} the experimental setup and {\bf b} the noise power spectrum from Rb vapor showing two peaks from $^{85}$Rb and $^{87}$Rb at corresponding Larmor frequencies. For more details, see Ref. \cite{noise-nat}. Reprinted with permission from Macmillan
Publishers Ltd: Nature 431, pp. 49–52, 2004, Copyright \copyright (2004) \cite{noise-nat}.
}
\label{noise-fig}
\end{figure}
\fi

The optical SNS is not restricted to
measurements of a single spin component or to fluctuations in
homogeneous spin systems. In such situations, one can consider
cross-correlations of spin densities with different indexes, e.g.,
\begin{equation}
%\begin{split}
C_{AB}(\om)=\int\limits_{-\infty}^{\infty}\textnormal{d}t\, e^{i\omega t}  \la S_A(t)S_B(0) \ra,
\label{cross-corr}
%\end{split}
\end{equation}
where A and B are indexes that may correspond to different atomic
species in an interacting gas mixture or  different spin
projections probed by noncollinear beams. Generally, the cross-correlator $C_{AB}(\om)$ is not
positive definite. Moreover, it can have both real and imaginary
components.

An example of the experimentally measured noise power spectrum is shown, e.g., in Fig.~\ref{noise-fig}(b). Typically, the spectrum consists of one or several peaks. Two types of peaks are most frequently encountered: the Lorentzian shaped peaks
\beq
C_{2}^L(\omega) \sim \frac{1}{(\omega-\omega_L)^2+\Gamma^2},
\label{lor-c2-1}
\eeq
and Gaussian shaped peaks
\beq
C_{2}^G(\omega) \sim e^{-\frac{\omega^2}{2\Gamma^2}},
\label{gauss-c2-1}
\eeq
where $\Gamma$ is a characteristic spin relaxation rate.
Performing the inverse Fourier transform, one can verify that, in the time domain, the Lorentzian shape corresponds to the exponentially damped spin precession
\beq
g_{2}^L(t) \sim e^{-\Gamma |t|} \cos(\omega_L t).
\label{exprel1}
\eeq
The Fourier transform of the Gaussian function remains the Gaussian one:
\beq
g_{2}^G(t) \sim e^{-\Gamma^2 t^2/2}.
\label{gauss-rel1}
\eeq
The exponential relaxation  (\ref{exprel1}) is usually associated with processes involving numerous fast mutually-uncorrelated microscopic interactions, such as atomic collisions, that contribute to the observed relaxation.
The relaxation according to the Gaussian law (\ref{gauss-rel1}) usually indicates the presence of dephasing processes, as in the case of an ensemble of similar systems with a Gaussian distribution of time-independent parameters.


\subsection{Higher Order Correlators}
A spin system's $n$-th order time-correlator is the average of a product of
$n$ results of the spin polarization measurements  taken at
different moments of time. The information content of 2nd order
correlators is intrinsically limited. Actually, this is not surprising as the noise power spectrum  tells us only
the weight of each frequency in the dynamics of spin
polarization without providing any information regarding correlations among different frequencies.
The complete information about an interacting spin system is contained in the full
set of all-order correlators \cite{2Dspectrum-mukamel}. Hence, the {\it higher order} SNS
is very interesting direction for future research.

 Higher order  correlators depend on more than one frequency, therefore, they are usually represented by multidimensional data, e.g. in the form of 2D or 3D density plots, that
contain additional and, possibly, considerably larger amount of
information about the system than the noise power spectrum  \cite{c4-1}. This information can be particularly useful when the studied spin
system experiences fluctuations at different time scales, such as in the case of a
qubit interacting with a slowly changing configuration of nuclear spins and simultaneously fast fluctuating spin-orbit fields due to interactions with phonons.
In other words,  higher order correlators are sensitive to the homogeneous broadening even in a strongly inhomogeneously broadened system,
i.e. they can be used to separate the effect of a static disorder from the intrinsic spin dynamics.

Another interesting property of higher order correlators is their intrinsic ``quantumness": Quantum measurements at intermediate time moments generally break the unitarity of evolution during the observed time interval. This fact may strongly influence higher order correlators, as it was demonstrated in a recent experiment \cite{alex-c3}, which extracted the quantum life time from an inhomogeneously broadened spectrum of a quantum dot spin qubit by using quantum properties of  the 3rd order correlator of spin projection operators.


% There is analogy here with
%music: the goal
%to understand spin interactions having only the knowledge of the 2nd
%order correlator is similar to the goal to reconstruct a melody knowing only how many times each note was played.
%\hl{[Not completely clear. If I am not mistaken, "how many times each note was played" is given by the Fourier spectrum, and 2nd order correlator
%provides information about the spacing between the notes.]}


To define higher order cumulants in the frequency domain,  let us introduce the normalized spin polarization
\begin{equation}
\delta S_z(t) = S_z(t)-\la S_z\ra,
\label{deltas}
\end{equation}
and consider its Fourier transform $a(\omega)$.  Similarly to the 2nd order correlator, in the steady state, only the products of $a(\omega_i)$ with $\sum_i \omega_i=0$ remain non-zero after the averaging. Hence, the next nearest nontrivial correlator of $a(\omega)$ is the 3rd order one  given by
\begin{equation}
C_3(\omega_1,\omega_2) = \langle a(\omega_1) a(\omega_2) a^* (\omega_1+\omega_2) \rangle.
\label{c3-1}
\end{equation}
A specific property of $C_3$ is that it is zero in a system with
time-reversal symmetry because spin variables are odd under the time reversal. Note also that the 3rd order correlator (\ref{c3-1}) is generally complex-valued.

 In the steady state, the 4th order cumulant is generally a
 function of three independent frequencies. Its definition depends on
 whether the sum of any two of these frequencies is zero or not. If the latter
 is the case, the 4th cumulant in the frequency domain can be defined as
 \begin{equation}
 C_4 (\omega_1,\omega_2,\omega_3) = \la   a(\omega_1) a(\omega_2) a(\omega_3) a^*(\omega_1+\omega_2+\omega_3) \rangle .
 \label{c4-1}
 \end{equation}
In the case of $ \quad \omega_1 =-\omega_3 \ne \omega_2$, the 4th order cumulant is defined as
\begin{equation}
 C_4 (\omega_1,\omega_2) \equiv \langle |a(\omega_1)|^2 |a(\omega_2)^2| \rangle -  \langle |a(\omega_1)|^2  \rangle \langle |a(\omega_2)^2| \rangle.
 \label{c4-11}
 \end{equation}
 Note that (\ref{c4-11}) cannot be obtained as a special case of (\ref{c4-1}).  The choice of the form of cumulants at equal values of some frequency parameters  is dictated by the requirement that such cumulants should be zero for Gaussian fluctuations of $a(\omega)$, so that the higher order cumulants do not duplicate the information that can be obtained from the lower ones.
 The correlators that depend on two frequencies, such as the 3rd order correlator (\ref{c3-1}) or the correlator (\ref{c4-11}), are often called the {\it bispectra}. A bispectrum  indicates how spin noise components at two different frequencies ``talk" to each other. For example, if $C_4(\omega_1,\omega_2)$ is negative, one can conclude the presence of anti-correlations, i.e. the observation of a strong signal at one frequency means that another frequency is likely suppressed, etc. An illustrative example of the experimental measurement of the correlator (\ref{c4-11}) can be found in \cite{fuxiang-c4}. Moreover, for $\omega_1=\omega_2=-\omega_3 \equiv \omega$,  the 4th cumulant is given by:
\begin{equation}
 C_4 (\omega) \equiv  \langle | a(\omega)|^4  \rangle -  2\langle |a(\omega)|^2  \rangle^2.
\label{c4-2}
 \end{equation}

Finally, there is a generalization of the correlator (\ref{c4-11}) called the ``noise
of susceptibility'' \cite{susceptibility-noise,forth-corr-maj}. In the correlator
(\ref{c4-2}), the product of 4th order spin variables is averaged over
repeated time intervals of duration $T_m$.  Instead, one can
measure the noise powers, $|a(\omega_1)|^2$ and $|a_T(\omega_2)|^2$,  of {\it different} time intervals  separated
by a given duration $T$, e.g., $(t,t+T_m)$ and $(t+T,t+T+T_m)$. One can  then  consider their
product averaged over all such pairs of intervals with different
$t$, separated by time $T$:
\begin{eqnarray}
\chi^{(4)} (\omega_1,\omega_2|T) = \nonumber \\
\quad =\la |a(\omega_1)|^2
|a_{T}(\omega_2)|^2\ra -\la |a(\omega_1)|^2 \ra \la |a_T(\omega_2)|^2 \ra.
\label{chi4}
\end{eqnarray}








\section{Survey of Experimental Results and Systems}
\label{exp}


%Experimental SNS techniques and history of their development have been extensively reviewed recently. Here, for completeness, we provide only a brief list of experimental results with a focus on goals and basic findings, while dropping technical details.

%From our theorist's perspective,
%Experimental research on spin noise can be classified in three
%types.

\subsection{Hot Atomic Vapors}

Hot atomic vapors are usually evaporated gases of atoms, such as K, Rb, Cs, above the room temperature (e.g., at 400K).
Atoms in a hot vapor are relatively energetic, so that
the average occupancy of states in these vapors is small ($\ll 1$).
In this regard, hot atomic vapors are different from ultra-cold gases, in which atoms tend
to occupy the lowest energy levels.

Hot atomic vapors have broad applications in magnetometry and isotope
separation techniques \cite{magnetometry-book,isotope-book}. As spin
fluctuations limit the precision of these applications,
future advances in these fields will likely depend on our
understanding of  spin noise  and our ability to control it. In fact, strategies to suppress unwanted spin fluctuations
by a feedback control have been recently demonstrated \cite{atomic1,atomic2}.
We also mention that a random number generator based on the atomic spin noise was recently proposed  \cite{random-number-gener}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
\centerline{\includegraphics[width=0.9\columnwidth]{fig3_1_2D-spectrum}}
%\includegraphics[width=2in]{two-color-fig.pdf}
\caption{Spin noise spectroscopy of $^{41}$K vapour subjected to a dc and weak ac
magnetic fields. (a) The measurement setup. (b)  The equilibrium noise power
    spectrum of $^{41}$K atomic vapor ($B_{ac}=0$). (c) The density plot of the noise power
  spectrum vs frequency of an ac-magnetic field applied in the transverse to
  the measurement beam direction. Simultaneous response of more than
  one peak to such external perturbation reveals cross-correlations
  between different spin resonances.
  Reprinted figure with permission from P. Glasenapp, et al.,
  Physical Review Letters 113, p. 156601, 2014 \cite{crooker-noneq1}.
  Copyright \copyright (2014) by the American Physical Society.}
\label{ac-SNS}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Equilibrium SNS.}  The nowadays interest in spontaneous spin fluctuations at the thermodynamic equilibrium originates from
the pioneering  experiments on Rb and K atomic vapors \cite{noise-nat}. These experiments clearly
resolved spin noise power peaks (Fig.~\ref{noise-fig}(b)) and explored the strategies for
digital signal processing. The noise power peaks were associated with resonances of
hyperfine coupled electronic spins.  This work has clearly demonstrated that spin interactions can be studied
at the thermodynamics equilibrium without externally exciting a system.

%Let's consider the interpretation of the noise power spectrum of a hot atomic vapor. For this purpose, we
Consider the atomic vapor of $^{41}$K that was investigated by SNS in Refs.~\cite{crooker-06pra2,crooker-06pra}.
Figure~\ref{ac-SNS} shows the experimental setup and the equilibrium noise power spectrum of this vapor measured in the applied magnetic field.
The spectrum consists of four Lorentzian peaks centered at different frequencies.

In $^{41}$K atoms, the uncompensated electronic spin with $S=1/2$ couples relatively strongly with a nuclear spin of $I=3/2$. The eigenstates of the exchange Hamiltonian $\hat{H}_0=\hat{\bf S}\cdot \hat{\bf I}$ split into two multiplets with the total angular momentum $F=1$ and $F=2$. The hyperfine splitting between the two multiplets is about 254 MHz, which is much higher than the frequency range of the spectrum shown in Fig.~\ref{ac-SNS}(b). The external magnetic field ${\bf B}=B\hat{y}$  modifies the Hamiltonian: $\hat{H}\approx \hat{H}_0 + g{\bf B}\cdot \hat{\bf S} $. Figure~\ref{ls} shows that the magnetic field ${\bf B}$ splits each multiplet into energy levels characterized by the projection of the total angular momentum $M$ on the field axis. Different pairs of nearest levels generally
experience a different size of splitting. We also note that the temperature of the atomic gas $T\sim 400K$ is orders of magnitude higher than the splitting between any pair of energy levels in Fig.~\ref{ls}. Therefore, one can consider that these levels are occupied with equal probabilities.

Let us assume that the measurement axis is transverse to the magnetic field direction as shown in Fig.~\ref{ac-SNS}(a). The optical beam couples to the electron spin  operator $\hat{S}_z$ that has nonzero matrix elements only between the pairs of states with $\Delta M =\pm  1$, where $M$ is the angular momentum projection on the magnetic field axis. The spin-spin correlator in real time can then be estimated as
\bea
\nn \la S_z(t)S_z(0) \ra &\sim &\sum_{i}  \la E_i| e^{i \hat{H}t}  \hat{S}_z  e^{-i \hat{H}t} \hat{S}_z |E_i\ra = \\
 &=&\sum_{i; j=i\pm 1} e^{i(E_j-E_i)t -\gamma_{ij} t  }|\la E_i|\hat{S}_z|E_j\ra|^2,  \label{SNPS2}
\eea
%\end{widetext}
where $E_j$ are the energies of the levels and index $i$ runs through all states. Note that in Eq.~(\ref{SNPS2}), for each resonance with the energy difference $E_j-E_i$, we introduced a phenomenological relaxation rate $\gamma_{ij}$.

Equation~(\ref{SNPS2}) shows that each pair of adjacent energy levels within each multiplet in Fig.~\ref{ls} contributes to the correlator with a damped oscillatory term $\sim e^{-\gamma_{ij}t} \cos([E_i-E_j]t)$.
After taking the Fourier transform, each such a term produces a Lorentzian peak in the noise power spectrum centered at $\omega = |E_i-E_j|$ (for $\omega>0$) with the width determined by the relaxation rate $\gamma_{ij}$.
Hence, the positions of these peaks can be used to find characteristic splittings between the energy levels, while their widths can be used to extract the relaxation rates. Moreover, Eq.~(\ref{SNPS2}) shows that the amplitudes of the peaks contain information about the matrix elements $\la E_i|\hat{S}_z|E_j\ra$.
\begin{figure}
\begin{center}
\includegraphics[width=0.65\columnwidth]{fig3_2_levelscheme}
\end{center}
\caption{4$^2$S$_{1/2}$ level diagram for $^{41}K$ atom in a constant magnetic field.}
\label{ls}
\end{figure}


Finally, we note that energy splittings between the levels with $M=0,1$ for $F=1$ and $F=2$, as well as between the levels with $M=-1,0$ for $F=1$ and $F=2$, are degenerate. This explains the only four peaks observed in Fig.~\ref{ac-SNS}(b) instead of six peaks as Fig.~\ref{ls} suggests.
Consequently, each of the two central peaks in Fig.~\ref{ac-SNS}(b) is the result of the overlap of two peaks from different resonances. This partly explains the relatively high amplitudes of the central peaks.

Relative heights of the peaks and
their behavior in external fields in relation to the matrix
elements of the measured electronic spin operator at different moments of time
were discussed in \cite{crooker-06pra2,crooker-06pra}. In
\cite{Katsoprinakis07}, an SNS-based approach to high precision relaxation time
measurements was developed.
In \cite{PhysRevA.84.043851}, the effect of the probe beam frequency on the spin
noise spectrum was explored. Peculiarities of near the resonance response were
attributed to collective effects.  Atomic gases were also used
as a simple testbed to improve SNS instrumentation
\cite{PhysRevLett.104.013601} and to demonstrate extensions of
this technique \cite{fuxiang-c4,crooker-13prl}.


Experiments with hot atomic gases are relatively simple. They do not require  cryogenic
equipment. Statistical filtering of physical spin correlators from the background noise in hot atomic gases,
such as $^{41}$K, can be achieved within few seconds. Moreover, the
electronic quantum states of different atomic isotopes have  been extensively studied by atomic physicists
throughout the 20th century and can be considered very well
understood. Due to this simplicity,  a methodology to teach the basics
of SNS in undergraduate laboratories was proposed in \cite{education}.
Hot atomic vapors are also
ideal for testing new measurement approaches and producing artificially correlated spin systems. Below, we discuss a few such
examples.



\subsubsection{Two-Color Spectroscopy.}
Electron spins cannot be generally considered identical even in the
same observation region. They can be localized near different
impurities, inside different quantum dots, etc. There are numerous
natural and engineered systems in which interactions between ``spins
of different kind" are important. Examples include the Kondo-lattices in correlated-electron materials \cite{heavy-fermions1, heavy-fermions2}, decoherence of solid-state spin qubits by a nuclear spin bath \cite{nuclear-bath1, nuclear-bath2, nuclear-bath3, Li12}, ferromagnetism in diluted magnetic semiconductors \cite{DMS1, DMS2}, and spin-exchange pumping of noble gas nuclei for medical imaging \cite{exchange-pumping}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
\centerline{\includegraphics[width=0.99\columnwidth]{fig3_3_two_col}}
\caption{Two probe beams measure fluctuations of spins of
  different atomic species. Cross-correlations between
spin fluctuations of different spin species provide information
regarding interactions between these different types of spins.
  Reprinted with permission from Macmillan Publishers Ltd:
  Scientific Reports 5, article number: 9573, 2015, Copyright \copyright (2015) \cite{two-color-2}.}
\label{two-color}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In \cite{two-color-2},  cross-correlations between spins of different kind were effectively
characterized by multi-probe SNS. The idea of this experiment is shown schematically in
Fig.~\ref{two-color}, wherein two atomic vapors, Cs and Rb,   interact
by the direct spin exchange at the thermal equilibrium. In this experiment, the spin fluctuations
from Cs and Rb are independently detected, and signatures of
spin interactions are observed in the cross-correlator (\ref{cross-corr}) of these two spin
noise signals. The authors of \cite{two-color-2} have demonstrated
that the spin relaxation and spin exchange rates can be measured
separately without ever perturbing the gas mixture from
the thermodynamic equilibrium.


\subsubsection{Beyond Equilibrium and Linear Response.}
One of the central results in statistical physics -- the fluctuation-dissipation theorem -- tells us that the information provided by the 2nd order correlators taken at the thermodynamic equilibrium is equivalent to the information that can be obtained by measuring a macroscopic linear response characteristic, such as the spin susceptibility. In this sense, the 2nd order correlator of spin fluctuations at the thermodynamic equilibrium does not provide any new information compared to the information that can be obtained, e.g., by the well developed pump-probe technique \cite{Young02a}, at least in principle.

However, the 2nd order correlator measured at {\it nonequilibrium} conditions is generally independent of the linear response characteristics.
The authors of \cite{crooker-noneq1} have explored the spin noise in the presence of a weak
radio frequency magnetic field, which was transverse both to the measurement and constant field axes.
This work demonstrated the possibility of a {\it multidimensional} SNS \cite{2Dspectrum-mukamel,2Dspectrum-2}, in which
the noise  power spectrum is represented as a function of both intrinsic and
driving field frequencies in a 2D density plot (as an example see Fig.~\ref{ac-SNS}(c)).  Such multidimensional
data show underlying patterns of correlations between different
frequencies and reveal numerous effects at the fluctuation level beyond the equilibrium and linear
response.

The multidimensional plots, such as Fig.~\ref{ac-SNS}(c), can be interpreted within the so called ``dressed state" Hamiltonian
\beq
\hat{H}_{\rm d}=\hat{H}+\hat{H}_{\rm EM}+\hat{V}
\label{ham-d}
\eeq
that describes the interaction of an atom with a coherent state of the electromagnetic field. Here $\hat{H}$ is the unperturbed atomic Hamiltonian, $\hat{H}_{\rm EM}$ is the secondary quantized Hamiltonian of the magnetic ac-field
\beq
\hat{H}_{\rm EM}=\omega_{ac} \hat{a}^{\dagger} \hat{a},
\eeq
where $\hat{a}^{\dg}$ and $\hat{a}$ are the creation and annihilation operators of the photons corresponding to this field mode, and
\beq
\hat{V}=\sum_{i} \tilde{\mu}_{i}B_{ac} (|E_i \ra \la E_{i+1}  | (\hat{a}+\hat{a}^{\dagger})+\textnormal{h.c.})
\label{ham-v}
\eeq
is the term describing the coupling of the radio frequency field of the amplitude $B_{ac}$ to the atomic spin states.

The electron spin-spin correlator of such a  system can be calculated similarly to Eq.~(\ref{SNPS2})
with the only difference that the index $i$ runs now throughout the eigenstates of the total Hamiltonian  (\ref{ham-d}).
For a weak ac-field, the interaction term (\ref{ham-v}) can be treated as a perturbation. In the first order in $\hat{V}$, the off-resonance values of the ac-field do not influence the spectrum.  However, if $\omega_{ac}$ is in resonance with any of the peaks then the corresponding peak splits into the so-called Mollow triplet \cite{Mollow69a} of three peaks. Moreover, if such a resonance shares a quantum level with another resonance, the latter also splits in the so-called
Autler-Townes doublet \cite{Autler55a} of two peaks. The distance between such splitted peaks is linear in the ac-field amplitude, $B_{ac}$. Higher ac-field amplitude leads to clearly observable nonlinear effects in the noise power spectrum, such as the appearance of the spin noise power peak centered at $\omega=\omega_{ac}$, additional splittings of other peaks, shifts of their positions, etc.  \cite{crooker-noneq1}.

The theory of dressed states is very well developed and cannot be reviewed here in detail. Fortunately, fairly complete and comprehensive introductions into this topic already exist (we refer to Refs.~\cite{budker-book,dressed-state-book} for further information). It should be emphasized that the importance of the work  \cite{crooker-noneq1} stems from the fact that for the first time  the rich physics of dressed states was observed at the fluctuation level without applications of pump laser pulses \cite{crooker-noneq1}.

The experimental demonstration of spontaneous spin fluctuations under steady nonequilibrium
conditions in atomic vapors \cite{crooker-noneq1} was followed by several theoretical studies
suggesting a broad range of applications for  {\it non-equilibrium} SNS.
In particular, it was proposed to use an ac-magnetic driving to
identify spin relaxation rates when the spin noise power spectrum is inhomogeneously broadened
(the quantum dots case) \cite{PhysRevB.91.155301}. In the case of electronic transport,
several effects (related to spin noise) were predicted both in the linear response regime
\cite{sinitsyn-13prl,sinitsyn-she} and far from equilibrium
\cite{golub-noneq}. The optical pumping can also be used to create nonequilibrium conditions. Spin noise of optically
induced exitons in semiconductors was explored theoretically in \cite{PhysRevB.90.085303}.


\subsubsection{Quantum Effects in Atomic Spin Noise.}
Squeezed spin states can be less susceptible to quantum
projection noise and thus can be used to increase the sensitivity of
magnetometers \cite{PhysRevA.50.67}. Experimental studies of quantum
projection noise and other spin fluctuations in such artificially
correlated atomic systems were reported in
\cite{projective-SNS,mitchel-12,mitchel-10,mitchel-11,polzik-01nat}.
The magnitude of artificially introduced correlations makes possible
observing their higher order spin cumulants experimentally \cite{Dellis13}.


We anticipate numerous applications of the optical SNS in atomic Bose-Einstein condensates and other ultracold atomic and molecular systems.
Currently, however, we are still at the very early stage in investigations of the  spontaneous equilibrium spin fluctuations in these systems using the optical
SNS. In fact, the proof-of-principle experiment was reported \cite{ultracold-noise}. This work communicates time-dependent spin fluctuations
in a cold atomic Fermi gas paying attention also to quantum measurement effects.

\subsection{Conduction Electrons in GaAs}

The first proof-of-principle measurements of the noise power spectrum of
conduction electron spins in GaAs revealed a much weaker useful signal in
comparison to atomic gases \cite{Oestreich05}. Nevertheless,
considerable improvements at the instrumentation and software levels \cite{gaas4,noise-gaas,ultrafast-sns} have
quickly enabled numerous SNS applications:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
\centerline{\includegraphics[width=0.9\columnwidth]{fig3_4_noise-T}}
\caption{The integrated noise power $P_{\rm int}=\int C_2(\omega) \textnormal{d}\omega$
  of electronic spins in GaAs as a function of temperature. Linear
  scaling is in good agreement with predictions of the Fermi liquid
  theory. A finite offset, however, indicates either localization
  effects or the presence of other spin noise sources in the sample.
  Reprinted figure with permission from S. A. Crooker et al.,
  Physical Review B 79, p. 035208, 2009 \cite{noise-gaas}.
  Copyright \copyright (2009) by the American Physical Society.
  }
\label{noise-T}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{itemize}

\item The temperature-dependent spin relaxation rate and the Lande $g$-factor at the
thermodynamic equilibrium were studied in \cite{noise-gaas}. The dependence of the spin noise power spectrum on the
doping concentration level was explored in \cite{gaas3,gaas5}. The influence of optical
excitations on  spin noise in semiconductors was investigated in
\cite{Huang2011}.

\item Measurements of  spin noise with {\it  picosecond } time resolution
were reported in \cite{high-band}. Such a {\it high
bandwidth spectroscopy} was used to observe  inhomogeneous broadening of
the spin noise peak of conduction electrons in a relatively large
magnetic field \cite{high-band}.

\item The inverse
Faraday effect \cite{inverse-faraday}, i.e. the appearance of an effective magnetic
field induced by a circularly polarized light, was observed at the spin
noise level \cite{impurity-noise-3,inverseFR-SNS}. These articles also report the
observation of a slow evolution of the noise power spectrum of
electrons interacting with polarized nuclear spins.

\end{itemize}

Spin dynamics of conduction electrons in $n$-doped materials has been relatively well
understood prior to the appearance of SNS.
However, some features of  spin noise in GaAs are still obscure. One such
observation \cite{noise-gaas} concerns the behavior of the
integrated noise power, $P_{\rm int}=\int P(\omega) \textnormal{d}\omega$, as function of
temperature $T$. The Fermi liquid theory predicts its linear
scaling $P_{\rm int}\sim T$ at low temperatures. However, the experiment \cite{noise-gaas} showed rather a linear scaling
with an offset, $P_{\rm int}= a+bT$, where $a$
and $b$ are constants (Fig.~\ref{noise-T}). The origin of this offset is not quite
understood. It can be due to the conduction electron localization or presence of deep
donor bound states.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
\centerline{\includegraphics[width=0.99\columnwidth]{fig3_5}}
%\includegraphics[width=2in]{two-color-fig.pdf}
\caption{Spin noise from a single GaAs quantum well embedded
into a microcavity \cite{Poltavtsev14}. (a) Measured noise
  power spectrum of conduction electrons. (b) Predictions of the
  theoretical model in \cite{Poltavtsev14} that includes exciton effects.
  Reprinted figure with permission from S. V. Poltavtsev et al.,
  Physical Review B 89, p. 081304, 2014 \cite{Poltavtsev14}.
  Copyright \copyright (2014) by the American Physical Society.
  }
\label{zero-peak1}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Another not fully explained feature of the noise power
spectrum is a small peak centered at zero frequency that persists even
in presence of an in-plane magnetic field (Fig.~\ref{zero-peak1}). The
magnetic field shifts most of
the noise power to the major Lorentzian peak centered at the Larmor frequency but
a small fraction of the noise power remains peaked at
$\omega=0$. Different explanations of this phenomenon have been
proposed. For example, a
small ellipticity of the probe beam polarization can lead to the
inverse Faraday effect \cite{inverse-faraday}, which does lead to a zero frequency
peak \cite{impurity-noise-3}. Another possible explanation is the presence of localized
states, which contribution to the spin noise power is usually centered
at zero frequency at weak external fields \cite{Crooker10}. There
has also been a proposal to relate this effect to excitons \cite{Poltavtsev14}.







% Moreover, such studies have revealed a number of unexpected effects that still remain poorly understood.


An important future goal is to extend  SNS to conduction electrons
in other materials. New measurement schemes have been proposed to increase the useful
signal-to-background ratio \cite{real-time-SNS,greilich-13,squeezed-15}. A big step in this
direction was an experiment on placing a 2D electron system in a
microcavity that considerably enhanced  coupling of the probe beam
to spins of conduction electrons \cite{Poltavtsev14}. This geometry
increased the useful signal by orders of
magnitude and allowed studies of spin noise from only a few hundreds of
electrons instead of millions in early experiments. Such micro-cavities can also be used to produce  strongly correlated  spin-photon states, which can be revealed by  spin noise measurements \cite{cavity-noise}.



%Theoretica studies of spin noise of itinerant electrons have

%Effects of interactions with the optical beam were explored in \cite{{gaas1}.
%  Lande g-factor and its anisotropy and electronic
%spin life-time at thermodynamic equilibrium were reported in \cite{PhysRevB.84.041301}
%gaas5,
%. so that spin noise studies in GaAs and
%heterostructures based on this material i

%Measurements of equilibrium spin noise were demonstrated at LANL and used to determine the g-factor, spin coherence and spin relaxation time in GaAs \cite{noise-gaas}.
%Other groups performed additional experimental studies of spin noise of conducting electrons in GaAs
%\cite{gaas1,gaas2}



%has improved data aquisition rate by four orders of magnitude
%\cite{noise-dots-prl} since the first experiments in 2005 \cite{noise-nat}.

\subsection{Quantum Dots}

Prior to the advances in SNS, the experimental studies of decoherence and
relaxation of quantum dot spin qubits
could not verify numerous theoretical predictions.
Earliest applications of the
SNS to hole-doped InGaAs quantum dots showed a relatively strong
useful signal per spin
\cite{Crooker10,ingaas-2}. Subsequent studies of the spin noise power
spectrum of quantum dots  have not only verified some of the theories
but also revealed some unexpected behavior. It was clearly demonstrated that
 SNS is capable of resolving  important questions
in materials science and uncover new physical phenomena.


When GaAs samples are grown with an admixture of indium atoms that
substitute gallium, indium does not disolve in the lattice uniformly
but rather creates InAs ``droplets'' of a few tens of nm
diameter and several nm height (shown in Fig.~\ref{fig3_6}(a)), which are called the self-assembled
quantum dots (QD). QDs provide a confining potential for a
localized single electron or hole state with an uncompensated spin.

In a relatively strong in-plane magnetic field, the spin noise power
spectrum  of hole-doped QDs was found to be in a good agreement with
theoretical expectations \cite{Crooker10}.  The spectrum consists of a shallow Gaussian
peak, which indicates the presence of the Larmor precession with
a strong inhomogeneous broadening due to different values of the
Lande $g$-factor of hole spins in different QDs. Moreover, the measured
anisotropy of the $g$-factor was in a good agreement with theoretical predictions
\cite{Crooker10}.  At zero magnetic field but relatively high temperatures, $T>7$K,
the experimental observations also agreed well with a theoretical expectation of
phonon-induced spin relaxation \cite{Li12}. It was found that at lower
temperatures, $T<7$K, the spectrum  no longer depended on $T$, which ruled
out the phonon origin of spin  relaxation and indicated
the transition to the regime where the spin relaxation was dominated by the coupling
to the nuclear spin bath.


\begin{figure}
\centerline{\includegraphics[width=0.99\columnwidth]{fig3_6}}
%\includegraphics[width=2in]{two-color-fig.pdf}
\caption{Spin noise from holes coupled to nuclear spin baths in (In, Ga)AS quantum dots \cite{Li12}.
(a) Experimental setup, (b) typical spin
noise power spectrum of the resident holes at a low temperature
(5 K) and zero applied magnetic field ($B=0$), and (c) the same spectrum on a log-log
scale. The noise line shape closely follows a Lorentzian, indicating
exponentially decaying hole spin correlations \cite{Li12}.
  Reprinted figure with permission from Y. Li et al.,
  Physical Review Letters 108, p. 186603, 2012 \cite{Li12}.
  Copyright \copyright (2012) by the American Physical Society.
  }
\label{fig3_6}
\end{figure}

An unexpected behavior was observed at $B=0$
and low temperature. It was found that the spectrum of hole-doped QDs
consists  of a single  narrow
Lorentzian peak (Fig.~\ref{fig3_6}(b)), indicating an exponential relaxation of hole spins
within $\sim 0.4$~$\mu$s \cite{Li12,ingaas-1}. To understand
why this behavior was unexpected, consider the  Hamiltonian that
describes the hyperfine coupling of the central spin  to a nuclear spin bath:
\begin{equation}
\hat{H}^{\rm hf} = \sum_{i=1}^N g^i_{||} \hat{S}_{z}
\hat{s}^i_{z}+\sum_{i=1}^N g^i_{\perp} (\hat{S}_{x}
\hat{s}^i_{x}+\hat{S}_{y}
\hat{s}^i_{y}),
\label{hole-ham1}
\end{equation}
where $\hat{S}_{\alpha}$, $\hat{s}^i_{\alpha}$  are the components of
the central and nuclear spin operators, respectively, $g^i_{||}$ and
$g_{\perp}^i$ are the out-of-plane and in-plane hyperfine
coupling constants describing the central spin and $i$th nuclear
spin interaction. Typically, the number of nuclear spins in an InGaAs quantum dot is $N\sim
10^5$. The hyperfine coupling is almost isotropic for electron-doped QDs
with $\la g^i \ra  \sim 1$ MHz. It is usually an order of magnitude smaller and
has a relatively strong out-of-plane anisotropy for
hole-doped QDs: $g_{\perp}^i/g_{||}^i \sim 0.2-0.5$.

Due to the large number of nuclear spins, one can justify the mean field
approximation, in which  the effect of the nuclear spin bath on the
central spin is described by an effective field, called the Overhauser
field $ {\bf B}_{\textnormal{O}}$ \cite{merkulov}:
\begin{equation}
\hat{H}_{\rm eff}^{\rm hf} = {\bf B}_{\textnormal{O}}\cdot \hat{\bf S}.
\label{over1}
\end{equation}
One can assume that this field points in a random direction, which is different in
different QDs. The components of the Overhauser field are
described by the Gaussian distribution, such that $\sqrt{\la B_{\textnormal{O},z}^2 \ra}  \sim g_{||} \sqrt{N}$ and $\sqrt{\la B_{\textnormal{O},x}^2 \ra },\sqrt{\la B_{\textnormal{O},y}^2 \ra } \sim g_{\perp} \sqrt{N}$.


\begin{figure}
%\centerline{\includegraphics[width=0.99\columnwidth]{broad-dots-fig.pdf}}
\includegraphics[width=3in]{fig3_7_broad-dots-fig.pdf}
\caption{ (a) The expected spin noise power spectrum  for a single quantum
  dot (as follows from Eq.~(\ref{dots-power})). (b) Inhomogeneous
  broadening of the finite frequency peak in an ensemble of quantum dots. }
\label{broad-dots}
\end{figure}
The size of the Overhauser field sets the frequency of precession of the
central spin around this field: $\omega_\textnormal{O}\approx g_{||} \sqrt{N} \sim
10$ MHz for hole-doped QDs. Let $\theta$ be the angle between
the Overhauser field and the measurement $z$-axis. A coherent spin polarization
precession around such a field is described by the correlator
\begin{equation}
\la S_z(t) S_z(0) \ra = \cos^2(\theta)+\sin^2(\theta) \cos(\omega_\textnormal{O} t),
\label{prec}
\end{equation}
where we normalized the correlator to 1 at $t=0$. While the spin polarization component
along the measurement axis remains constant, the other
part oscillates \cite{merkulov}. The Fourier transform
of this correlator produces two delta-functions (Fig.~\ref{broad-dots}(a)): one at zero frequency and another
at $\omega_\textnormal{O}$:
\begin{equation}
P(\omega)\equiv C_2(\omega) = \cos^2(\theta)\delta(\omega) +\sin^2(\theta) \delta(\omega-\omega_\textnormal{O}).
\label{dots-power}
\end{equation}

If  measurements are performed on an ensemble
of a large number of quantum dots, Eq.~(\ref{dots-power}) should be
averaged over the distribution of the Overhasuer field. Each quantum dot
then still contributes to the $\delta$-function at $\omega=0$ and, in addition,
produces a finite frequency contribution at its individual $\omega_\textnormal{O}$, so
that the high frequency peak is expected to be broadened and have the
Gaussian shape, as shown in Fig.~\ref{broad-dots}(b). The maximum of this peak is expected to be at $\omega \approx
g_{||} \sqrt{N} \sim 10$ MHz. There have been debates in theoretical
literature about the role of the slow dynamics of the Overhauser
field. This dynamics is responsible for the broadening of the zero
frequency peak. Numerical studies \cite{dobrovitski,Faribault2013,sinitsyn-12prl-2}  have shown that, within the model
(\ref{hole-ham1}), this dynamics is very slow so that only a small power-law broadening
of the zero frequency peak is expected, not exceeding the transverse hyperfine
coupling frequency scale $g_{\perp} <0.1$ MHz.


Apparently, the experimental observation \cite{Li12} of a single Lorentzian peak with a
width of $\sim 1$ MHz (Fig.~\ref{fig3_6}(b)) strongly contradicts the above
expectation. Not only the shape of the peak but also
its characteristic width could not be explained by the above mentioned theory. Moreover, this result can
not be related to an unusual inhomogeneous broadening.
In fact, it was possible to make an experiment in
which all but one quantum dots were  shielded from the probe beam so
that the Faraday rotation noise spectrum of a {\it single spin} was detected
\cite{single-spin}. At zero magnetic field, no deviations in measurement
results for a single quantum dot from the results for an ensemble of quantum dots
were found.

%The reason is that if quantum dots are well separated from each other,
%spins from different dots produce statistically independent
%contributions to the measured noise power spectrum.


The experimental observations reported in \cite{Li12,ingaas-1} were
explained theoretically in Ref.~\cite{sinitsyn-12prl-2} by the presence
of quadrupole couplings, whose importance had been clearly exposed
earlier in Ref.~\cite{imamoglu-quad}. A more realistic Hamiltonian is written as
\begin{equation}
 \hat{H}= \hat{H}^{\rm hf}+ \sum_{i=1}^N \frac{\gamma_q^i}{2} (\hat{\bf s}^i \cdot {\bf n}^i)^2 ,
\label{Ham-q}
\end{equation}
where $\hat{H}^{\rm hf}$ is defined by Eq.~(\ref{over1}), $\gamma_q^i$ is
the strength of the quadrupole coupling of the $i$th nuclear spin, $\hat{\bf s}^i$ is the nuclear spin operator, and
${\bf n}^i$ is the unit vector along the direction of the local quadrupole coupling anisotropy.
The last term in Eq.~(\ref{Ham-q}) becomes nontrivial, i.e., different from a constant when $s^i>1/2$. In fact,
the most abundant isotopes of Ga and In are characterized by
$s=3/2$ and $s=9/2$, respectively.
The assumption \cite{sinitsyn-12prl-2} of a broad distribution of ${\bf n}^i$  inside
self-assembled quantum dots helped to explain the experimental observations.

An analytical solution to the system described by the Hamiltonian (\ref{Ham-q}) can
be found in the limit of a large quadrupole coupling, which is
relevant to the hole-doped dots. In this case, the nuclear spin dynamics
is dominated by the last term in (\ref{Ham-q}), which induces fluctuations of the
Overhauser field with a typical amplitude $\sim g_{||} \sqrt{N}$ and
correlation time $\sim \gamma_qs/2$.  The dynamics of the central spin subjected to
such a fluctuating Overhauser field was investigated in
\cite{sinitsyn-12prl-2}, where it was shown that in hole-doped InGaAs
quantum dots the central spin  relaxes exponentially. In the case of electron-doped dots, numerical simulations
\cite{sinitsyn-12prl-2,electron-dot} predict that the basic
physics leading to Fig.~\ref{broad-dots}(b) is correct except the
zero frequency peak is broadened by the quadrupole coupling effects.  This difference from the hole-doped quantum dots follows mainly from order of magnitude stronger hyperfine coupling, which reduces the relative role of the quadrupole coupling effects. Recent optical measurements of spin correlators in electron-doped dots \cite{alex-nat,electron-dot}  and spins confined near impurities \cite{impurity-noise-3} have confirmed this prediction. Moreover,
experiments with a single quantum dot revealed an additional oscillation in the spin correlator in the time-domain,
which was also explained by the quadrupole coupling effect \cite{alex-nat}.


%So, if there is no
%big effect of inhomogenerou broadening, which is the case at zero
%external field, different spins produce statistically independent and similar
%contributions.



%\begin{figure}
%\centerline{\includegraphics[width=0.99\columnwidth]{fig3_7_singleQD}}
%\includegraphics[width=2in]{two-color-fig.pdf}
%\caption{Optical spin noise of a single hole spin localized in an (InGa)As quantum dot \cite{single-spin}.
%The blue squares depict the measured integrated spin noise power while the solid lines represent the photoluminescence
%spectrum for two orthogonal linear polarizations. Typical spin noise spectrum at a
%low magnetic field is exhibited in the inset.
%  Reprinted figure with permission from R. Dahbashi et al.,
%  Physical Review Letters 111, p. 156601, 2014 \cite{single-spin}.
%  Copyright \copyright (2014) by the American Physical Society.
%  }
%\label{fig3_7_singleQD}
%\end{figure}


%\subsubsection{Faraday spectroscopy of charge fluctuations.}



%\subsection{Other applications}
%There have been scattered reports of optical characterization of spin
%noise in various other systems.  Such developments raise the
%optimism in that the future scope of SNS applciations will be
%eventually much broader that it is today.

\subsection{Magnetic Impurities, Thin Magnetic Films, and  Nanomagnets}

The spin noise power spectrum of localized electrons bound to
impurities has been observed in \cite{PhysRevB.87.045312}.
The noise from such bound electrons is similar to the noise from electrons confined
in quantum dots. This is explained by the same spin relaxation mechanism at low temperatures:
the electron spin interaction with local nuclear spins. Importantly,  impurities have
a reproducible confining potential. Consequently, the resulting spin
noise is less influenced by inhomogeneous broadening, which can be
very strong in quantum dots.

The spin noise power measurements of magnetic Mn ions in CdTe quantum
wells were reported in \cite{mn-noise}. In this system, the spin noise
power spectrum has a relatively complex form explained by multiple resonances of spin-5/2  Mn ions.
%Some of the features of this spectrum could not be easily explained.
%This spectrum could be even more complex due to magnetic
%crystal anisotropy that splits some of the degeneracies but the
% broadening of noise power peaks in \cite{mn-noise} was likely too strong to
%allow resolution of such subtle details.

The authors of \cite{impurity-noise-3} have communicated the spin noise power spectrum
of electrons bound to Si impurities in GaAs.
The measured noise power spectrum contains two clear peaks - one centered at
zero and another one centered at the characteristic frequency of the Overhauser
field. The application of the external magnetic field removes the zero
frequency peak and produces a Gaussian broadened peak at the Larmor frequency, as expected.
The spin dephasing and relaxation times of electrons bound to Si impurities in GaAs are longer
compared to these in InGaAs quantum dots.

%\subsection{}

In \cite{balk2014critical}, the Kerr rotation spectroscopy was applied to
detect ferromagnetic fluctuations and random thermal motion of domain
walls in a thin film made of magnetic Co atoms.  The width of the film
varied so that  the magnetization fluctuations could be studied in different phases near the ferromagnetic phase transition. Due to the large size of the domain walls,  both temporal and
spatial noise characterization was performed.

In \cite{liu-echo}, the optical SNS was applied to study fluctuations of the magnetization in molecular nanomagnets. The latter are molecules with uncompensated spins of magnetic ions. Typically, spins of
nanomagnets experience magnetic crystal anisotropy, in which they have two or several degenerate ground states. This degeneracy is lifted by spin tunneling and interactions of nanomagnets with each
other and with nuclear spins. Fluctuations of the magnetization of nanomagnets can be used for precise parameter estimation of these technologically interesting nanostructures.


%\begin{figure}
%\centerline{\includegraphics[width=0.99\columnwidth]{fig3_8_quantum_gas}}
%\caption{
%Interferometric measurement of local spin-fluctuations in a quantum gas \cite{ultracold-noise}.
%The probe (passing through the cloud) and local oscillator (passing by the side) beams  overlap in
%the far field giving rise to an interference pattern as shown.
 % Reprinted with permission from Macmillan Publishers Ltd: Nature Physics 8, 454, 2012, Copyright \copyright (2012) \cite{ultracold-noise}.
 % }
%\label{fig3_8_quantum_gas}
%\end{figure}

\subsection{Alternative SNS Techniques}

Non-optical SNS methods usually do not
probe the spin polarization directly but rather detect fluctuations of
the local magnetic field produced by flipping spins. The sensitivity
of such techniques to the relative position of probe and noise
sources complicates the interpretation of the signal. At the same time,
this can be used as an advantage in situations when a better spatial resolution is needed.

{\it Barkhausen noise.} Studies of fluctuations in magnetic
systems take roots in the work of Heinrich Barkhausen who proved already in 1919
that the magnetic hysteresis curve is not continuous,
but is made up of small random steps caused when the magnetic domains
move under an applied magnetic field \cite{barkhausen}.
This noise can be characterized by placing a coil of a conducting wire
near the sample. Motion of ferromagnetic domain walls produces changes
in the magnetization that induces noisy electrical signals in the
coil. Studies of Barkhausen noise have been used in practice as a
nondemolition tool to characterize distribution of elastic stresses and the micro-structure of magnetic samples \cite{barkhausen-rev}.

{\it SQUID-based spectroscopy.} Superconducting quantum
interference devices (SQUIDs) have been the method of choice for
studies of magnetic field fluctuations in superconductors
\cite{PhysRevB.57.10929}, spin glasses \cite{PhysRevLett.57.905,
  PhysRevLett.57.905,PhysRevB.40.7162}, ferroelectric liquid crystals \cite{PhysRevLett.79.1062}, and nanomagnets
\cite{PhysRevB.57.497}.  In this approach,
the sample is placed directly in the vicinity of a dc-SQUID chip with integrated
pickup loops and field coils that detects magnetic field fluctuations
that originate from
flipping magnetic moments. The frequency bandwidth of SQUID devices is
relatively small in comparison to optical SNS setups. It is most
suitable for materials made of ferromagnetic grains or large spins, such as nanomagnet arrays.
Strong disorder, dipole interactions, and anisotropy fields lead to a
broad distribution of spin relaxation rates in such samples so that
the measured noise power spectra usually were reported to have the
form of $\sim 1/f$ or $\sim 1/f^{\alpha}$ noise. Yet, the dependence
of such spectra on temperature and the magnetic field could be used to
extract important physics. A number of theoretical publications have
been devoted to this field, e.g., to  the origin of the
power laws and violation of the fluctuation-dissipation theorem in
spin glasses
 \cite{PhysRevLett.113.217002,PhysRevLett.104.247204,PhysRevLett.83.5038,PhysRevB.86.134414}.


{\it Cantilever-based spectroscopy.}
 Local fluctuations of spins can  also be probed with a nanomechanical
 resonator \cite{cantilever-science,cantilever-noise}. In this approach,
 fluctuations of the magnetization are detected via measuring their
 mechanical force that the time-dependent spin polarization produces on a small permanent
 magnet attached to the end of a sensitive silicon
 cantilever. This technique was successfully applied to ensembles
 of electronic localized spins  \cite{cantilever-science},  molecular
 nanomagnets \cite{cantilever-noise}, and nuclear spins \cite{cantilever-NMR}. Currently, the
 allowed frequency bandwidth is comparable to the optical techniques,
 while cantilever-based spectroscopy has a better spatial resolution
 and is not restricted to optically sensitive materials. Its
 applications are restricted, however, to spins near the surface of a
 sample. Interpretation of the data can be complicated by complex
 distribution of forces with which spins at different locations act on
 the probe mechanical resonator.


{\it STM-based spectroscopy.}
Measuring fluctuations of a spin polarized tunneling current from an STM tip can
be used to extract spectroscopic information on the temporal
susceptibility of a single magnetic atom. This technique has an
exceptional time and atomic-scale spatial resolution. However, its applications are restricted to
 surface spins. Moreover, technical problems such as the lack of a good
control of the magnitude of the tunneling current
remain to be resolved. For a detailed discussion of this method, we refer the reader to a recent
 review \cite{balatsky-stm-rev} and theoretical papers \cite{balatsky-noise, PhysRevB.70.033405,PhysRevB.73.184429,PhysRevLett.102.256802}.

{\it X-ray photon correlation spectroscopy.}
This experimental technique
has been used for many different purposes including studies of
domain wall fluctuations in antiferromagnets at short wavelengths \cite{Shpyrko07a,Jacques14a}. In this application, a coherent beam
reflected from a sample surface (chromium (111) surface in Ref. \cite{Shpyrko07a}) creates an interference pattern known as speckle \cite{dainty1975laser,goodman1976some} (see Fig.~\ref{fig3_10_X_ray} for a speckle example).
The sensitivity of the speckle to the domain wall structure was used to obtain information regarding the microscopic dynamics of antiferromagnetic domains  \cite{Shpyrko07a}. In the speckle data analysis, the autocorrelation function $g_2(t)=\left< I(\tau)I(\tau+t) \right>_\tau /\left< I(\tau) \right>^2_\tau$ is found for a given pixel and used to extract relevant time scales. The theory of coherent light propagation in disordered media and speckle statistics was developed in \cite{andreev-speckles}.

The chromium antiferromagnetism is a complex phenomenon associated with spin- and charge-density waves of different periods. In Ref.~\cite{Shpyrko07a}, the spin-density wave dynamics was tested indirectly at a charge-density wave Bragg reflection angle. It's interesting that the reflection at the spin-density wave angle contains just a single stationary peak \cite{Jacques14a}. Therefore, we feel that there is a need of better understanding of
co-existence of the spin- and charge-density waves in chromium, and their coupling to light.

\begin{figure}
\centerline{\includegraphics[width=0.75\columnwidth]{fig3_8_X_ray}}
\caption{CCD image of the X-ray speckle observed for the chromium [200] lattice
Bragg reflection (for more details, see Ref. \cite{Shpyrko07a}).
Reprinted with permission from Macmillan
Publishers Ltd: Nature 447, pp. 68–-71, 2007, Copyright \copyright (2007) \cite{Shpyrko07a}.}
\label{fig3_10_X_ray}
\end{figure}

\subsection{Nuclear Spin Noise}
 The nuclear magnetic fields from mesoscopic volumes at equilibrium are extremely weak.
Nevertheless, it is possible to study
fluctuations of such fields \cite{nuclear-noise1,chandra2013spin}. For example,
SQUID probes were used to measure the nuclear spin noise as early as in 1985 \cite{nuclear-noise}.
An approach based on the STM tunneling spectroscopy was theoretically developed in \cite{PhysRevB.73.184429}.


A cantilever based
detector was used in \cite{cantilever-NMR} to resolve mesoscopic nuclear spin noise in real
time with submicron resolution.  This experiment not only allowed studies of nuclear spin diffusion but also demonstrated the capability
to manipulate the local nuclear spin distribution.


Considerable progress in the detection of nuclear spin noise has been
achieved recently using nanomagnetometry based on NV-centers in diamonds \cite{NV2,NV3,nV1}. Magnetic field
fluctuations, as small as 10nT, from a single nuclear spin have been resolved
with a nanometer precision \cite{NV4}. Electronic spins in
coupled GaAs quantum dots were also shown to work as a sensitive probe of the environmental field fluctuations \cite{yakoby-13prl}.

Finally, although optical beams do not couple to the nuclear spin
polarization directly, the noise power spectrum of nuclear
spins has been recently observed by optical SNS \cite{impurity-noise-3}. In
this experiment, the electronic spin noise in a silicon doped ultraclean GaAs
semiconductor was studied. Surprisingly, in addition to the expected
noise power peaks of donor-bound electrons, relatively weak peaks have
been observed in the low frequency (10-100kHz) range. Such peaks
responded to the
external magnetic field as expected from the nuclear spin noise of the  host isotopes: $^{75}$As, $^{69}$Ga and
$^{71}$Ga. This finding allowed the authors of
\cite{impurity-noise-3} to explore the nuclear spin noise at very low
magnetic field values and observe effects consistent with presence of quadrupole couplings.
Apparently, this feature in the optically probed noise power spectrum follows from fluctuations of local
Overhauser fields that nuclear spin fluctuations induce on observable electronic
spins, although detailed theory of this effect has not been developed.  It is possible, e.g., that a precessing nuclear spin polarization creates an effective ac-like Overhauser
field that can produce a noise power peak of electronic spins at
the precession frequency as a 2nd order effect in the field
amplitude \cite{crooker-noneq1}.



